How Well Do Text Embedding Models Understand Syntax?

Text embedding models have significantly contributed to advancements in natural language processing by adeptly capturing semantic properties of textual data. However, the ability of these models to generalize across a wide range of syntactic contexts remains under-explored. In this paper, we first develop an evaluation set, named \textbf{SR}, to scrutinize the capability for syntax understanding of text embedding models from two crucial syntactic aspects: Structural heuristics, and Relational understanding among concepts, as revealed by the performance gaps in previous studies. Our findings reveal that existing text embedding models have not sufficiently addressed these syntactic understanding challenges, and such ineffectiveness becomes even more apparent when evaluated against existing benchmark datasets. Furthermore, we conduct rigorous analysis to unearth factors that lead to such limitations and examine why previous evaluations fail to detect such ineffectiveness. Lastly, we propose strategies to augment the generalization ability of text embedding models in diverse syntactic scenarios. This study serves to highlight the hurdles associated with syntactic generalization and provides pragmatic guidance for boosting model performance across varied syntactic contexts.

==> Tables/Lexical.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Model}  & \textbf{STS-B}  & \textbf{CQADupStack} & \textbf{Twitter} &  \textbf{BIOSSES}  & \textbf{Avg} \\
\midrule
\midrule
\multicolumn{6}{c}{\textit{Lexical Compositionality}} \\
\midrule
\midrule
% SBERT-BERT-Base(training on stsb training) & 22.68 & - & - & - & - \\
% SBERT-BERT-Base(training on LSR training) & 37.43 & - & - & - & - \\
% SBERT-BERT-Large(training on stsb training) & 27.56 & - & - & - & - \\
% SBERT-BERT-Large(training on LSR training) & 41.20 & - & - & - & - \\
% SBERT-BERT-Base(training on stsb training) & 29.03 & - & - & - & - \\
% SBERT-BERT-Base(training on LSR training) & 42.36 & - & - & - & - \\
% SBERT-BERT-Base(training on stsb training) & 31.79 & - & - & - & - \\
% SBERT-BERT-Base(training on LSR training) & 43.39 & - & - & - & - \\
SimCSE-BERT-Base-sup & 32.77 & 5.01 & 17.86 & 40.06 & 23.92 \\
SimCSE-BERT-Large-sup & 33.29 & 4.49 & 17.55 & 40.74 & 23.99 \\
SimCSE-RoBERTa-Base-sup & 34.91 & 5.39 & 18.09 & 40.82 & 24.80 \\
SimCSE-RoBERTa-Large-sup & 38.24 & 6.59 & 19.64 & 42.69 & 26.79 \\
Sentence-T5-Base & 34.24 & 6.39 & 22.41 & 36.00 & 24.76 \\
Sentence-T5-Large & 36.11 & 6.61 & 21.61 & 38.79 & 25.78 \\
Sentence-T5-XL & 37.49 & 7.70 & 21.46 & 36.31 & 25.74 \\
Sentence-T5-XXL & 38.39 & 7.15 & 22.17 & 39.27 & 26.74 \\
Instructor-Base & 28.02 & 7.31 & 18.20 & 26.96 & 20.12 \\
Instructor-Large & 32.69 & 8.31 & 18.68 & 39.30 & 24.74 \\
Instructor-XL & 28.57 & 7.81 & 20.38 & 31.18 & 21.98 \\
OpenAI(text-embedding-ada-002) & 26.43 & 6.67 & 20.73 & 26.37 & 20.05 \\
\midrule
\midrule
\multicolumn{6}{c}{\textit{Structural Heuristics}} \\
\midrule
\midrule
SimCSE-BERT-unsup & 19.14 & 14.17 & 19.68 & 37.27 & 22.56 \\
SimCSE-BERT-sup & 19.93 & 15.60 & 18.59 & 35.13 & 22.31 \\
SimCSE-RoBERTa-unsup & 19.29 & 18.12 & 16.00 & 34.58 & 22.00 \\
SimCSE-RoBERTa-sup & 22.97 & 19.20 & 15.88 & 35.42 & 23.37 \\
Sentence-T5-base & 15.60 & 23.31 & 20.80 & 35.45 & 23.79 \\
Sentence-T5-Large & 17.03 & 24.30 & 21.83 & 35.90 & 24.77 \\
Sentence-T5-XL & 17.86 & 26.93 & 21.24 & 35.79 & 25.46 \\
Sentence-T5-XXL & 18.04 & 25.01 & 20.65 & 32.22 & 23.98 \\
Instructor-Base & 17.48 & 21.06 & 15.95 & 23.31 & 19.45 \\
Instructor-Large & 20.96 & 22.09 & 19.34 & 29.79 & 23.04 \\
Instructor-XL & 20.46 & 19.97 & 20.28 & 26.55 & 21.82 \\
OpenAI (text-embedding-ada-002) & 15.35 & 26.50 & 17.90 & 22.40 & 20.54 \\
\midrule
\midrule
\multicolumn{6}{c}{\textit{Relational Understanding}} \\
\midrule
\midrule
SimCSE-BERT-unsup & 30.39 & 30.15 & 38.07 & 41.79 & 35.10 \\
SimCSE-BERT-sup & 38.8 & 30.64 & 40.09 & 48.80 & 39.58 \\
SimCSE-RoBERTa-unsup & 28.2 & 26.23 & 36.32 & 45.00 & 33.94 \\
SimCSE-RoBERTa-sup & 48.34 & 31.28 & 40.22 & 50.43 & 42.57 \\
Sentence-T5-base & 33.61 & 35.72 & 42.53 & 47.63 & 39.87 \\
Sentence-T5-Large & 51.08 & 39.85 & 44.80 & 53.82 & 47.39 \\
Sentence-T5-XL & 58.64 & 42.10 & 48.21 & 53.41 & 50.59 \\
Sentence-T5-XXL & 60.3 & 42.35 & 49.69 & 54.52 & 51.71 \\
Instructor-Base & 1.33 & 31.46 & 36.75 & 18.68 & 22.06 \\
Instructor-Large & 21.88 & 38.50 & 40.71 & 41.74 & 35.71 \\
Instructor-XL & 28.97 & 39.30 & 42.34 & 35.24 & 36.46 \\
OpenAI (text-embedding-ada-002) & 19.10 & 24.60 & 33.20 & 29.90 & 26.70 \\
\bottomrule 
\end{tabular}

\caption{The evaluation result of LSR Benchmark . Spearman rank correlation $\rho$ between the cosine similarity of sentence representations and the  labels.}
\label{tab:main_results}
\end{table*}


==> Tables/Relational.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Model}  & \textbf{STS-B} & \textbf{CQADupStack} & \textbf{Twitter} &   \textbf{BIOSSES}  & \textbf{Avg} \\
\midrule    
% SBERT-BERT-Base(training on stsb training) & 13.45 & - & - & - & - \\
% SBERT-BERT-Base(training on LSR training) & 56.57 & - & - & - & - \\
% SBERT-BERT-Large(training on stsb training) & 24.95 & - & - & - & - \\
% SBERT-BERT-Large(training on LSR training) & 60.16 & - & - & - & - \\
% SBERT-BERT-Base(training on stsb training) & 11.87 & - & - & - & - \\
% SBERT-BERT-Base(training on LSR training) & 58.65 & - & - & - & - \\
% SBERT-BERT-Base(training on stsb training) & 26.93 & - & - & - & - \\
% SBERT-BERT-Base(training on LSR training) & 62.82 & - & - & - & - \\
SimCSE-BERT-unsup & 30.39 & 30.15 & 38.07 & 41.79 & 35.10 \\
SimCSE-BERT-sup & 38.8 & 30.64 & 40.09 & 48.80 & 39.58 \\
SimCSE-RoBERTa-unsup & 28.2 & 26.23 & 36.32 & 45.00 & 33.94 \\
SimCSE-RoBERTa-sup & 48.34 & 31.28 & 40.22 & 50.43 & 42.57 \\
Sentence-T5-base & 33.61 & 35.72 & 42.53 & 47.63 & 39.87 \\
Sentence-T5-Large & 51.08 & 39.85 & 44.80 & 53.82 & 47.39 \\
Sentence-T5-XL & 58.64 & 42.10 & 48.21 & 53.41 & 50.59 \\
Sentence-T5-XXL & 60.3 & 42.35 & 49.69 & 54.52 & 51.71 \\
Instructor-Base & 1.33 & 31.46 & 36.75 & 18.68 & 22.06 \\
Instructor-Large & 21.88 & 38.50 & 40.71 & 41.74 & 35.71 \\
Instructor-XL & 28.97 & 39.30 & 42.34 & 35.24 & 36.46 \\
OpenAI (text-embedding-ada-002) & 19.10 & 24.60 & 33.20 & 29.90 & 26.70 \\
\bottomrule 
\end{tabular}

\caption{The evaluation result of Benchmark For Assessing Relational Understanding. Spearman rank correlation $\rho$ between the cosine similarity of sentence representations and the  labels.}
\label{tab:main_results}
\end{table*}


==> Tables/Structural.tex <==
\begin{table*}
\centering
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Model}  & \textbf{STS-B} & \textbf{CQADupStack} & \textbf{Twitter} &   \textbf{BIOSSES}  & \textbf{Avg} \\
\midrule
% SBERT-BERT-Base(training on stsb training) & 18.15 & - & - & - & - \\
% SBERT-BERT-Base(training on LSR training) & 30.91 & - & - & - & - \\
% SBERT-BERT-Large(training on stsb training) & 19.62 & - & - & - & - \\
% SBERT-BERT-Large(training on LSR training) & 33.93 & - & - & - & - \\
% SBERT-BERT-Base(training on stsb training) & 16.90 & - & - & - & - \\
% SBERT-BERT-Base(training on LSR training) & 29.04 & - & - & - & - \\
% SBERT-BERT-Base(training on stsb training) & 19.38 & - & - & - & - \\
% SBERT-BERT-Base(training on LSR training) & 33.61 & - & - & - & - \\
SimCSE-BERT-unsup & 19.14 & 14.17 & 19.68 & 37.27 & 22.56 \\
SimCSE-BERT-sup & 19.93 & 15.60 & 18.59 & 35.13 & 22.31 \\
SimCSE-RoBERTa-unsup & 19.29 & 18.12 & 16.00 & 34.58 & 22.00 \\
SimCSE-RoBERTa-sup & 22.97 & 19.20 & 15.88 & 35.42 & 23.37 \\
Sentence-T5-base & 15.60 & 23.31 & 20.80 & 35.45 & 23.79 \\
Sentence-T5-Large & 17.03 & 24.30 & 21.83 & 35.90 & 24.77 \\
Sentence-T5-XL & 17.86 & 26.93 & 21.24 & 35.79 & 25.46 \\
Sentence-T5-XXL & 18.04 & 25.01 & 20.65 & 32.22 & 23.98 \\
Instructor-Base & 17.48 & 21.06 & 15.95 & 23.31 & 19.45 \\
Instructor-Large & 20.96 & 22.09 & 19.34 & 29.79 & 23.04 \\
Instructor-XL & 20.46 & 19.97 & 20.28 & 26.55 & 21.82 \\
OpenAI (text-embedding-ada-002) & 15.35 & 26.50 & 17.90 & 22.40 & 20.54 \\
\midrule
\midrule


\bottomrule 
\end{tabular}

\caption{The evaluation result of Benchmark For Assessing Structural Heuristics. Spearman rank correlation $\rho$ between the cosine similarity of sentence representations and the  labels.}
\label{tab:main_results}
\end{table*}


==> Tables/human.tex <==
\begin{table}
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Model}  & \textbf{Human} & \textbf{ChatGPT} & \textbf{Ensemble}  \\
\midrule
SBERT-bert-large       & 84.52      & 79.26   & 85.74    \\
SBERT-roberta-large   & 86.71      & 80.54   &87.58\\
\bottomrule
\end{tabular}

\caption{We employ Spearman's rank correlation coefficient to measure the alignment between ChatGPT annotations and those obtained  by text embedding models.  \textbf{Human:} standard STS-B test set,  \textbf{ChatGPT:} STS-B test set with scores annotated by ChatGPT, \textbf{ensembled:} ensembled test set of both human and ChatGPT annotations.}
\label{tab:prompt_ablation}
\end{table}


% \begin{table}
% \centering
% \small
% \begin{tabular}{lccc}
% \toprule
% \textbf{Method}  & \textbf{Human} & \textbf{ChatGPT} & \textbf{Ensemble}  \\
% \midrule
% \textbf{Human}       & -      & 83.8   & 96.5    \\
% \textbf{ChatGPT}   & 83.8      & -   &95.2\\
% \bottomrule
% \end{tabular}

% \caption{We employ Spearman's rank correlation coefficient to measure the alignment between human annotations and those generated by ChatGPT. \textbf{Human:} standard STS-B test set,  \textbf{ChatGPT:} STS-B test set with scores annotated by ChatGPT, \textbf{ensembled:} ensembled test set of both human and ChatGPT annotations.}
% \label{tab:prompt_ablation}
% \end{table}

==> backups/abstract.tex <==
\begin{abstract}
This work investigates the syntactic generalization capabilities of text embedding models and presents insights derived from a benchmark study. Text embedding models have significantly advanced natural language processing tasks by capturing semantic properties of textual data. However, their ability to generalize across diverse syntactic contexts  remains questionable. In this study, we introduce an evaluation  set to probe the ability of text embedding models in grappling with three syntactic dimensions: lexical compositionality, structural heuristics, and  relational understanding among concepts based on previous benchmarks.   We demonstrate that the existing text embedding models has not been enough to address the lack of syntactic understanding, and the evaluation of these models on past benchmark datasets has proven inadequate in identifying this particular limitation.  Furthermore, we conduct an analysis to uncover insights into the factors contributing to the manifestation of these limitations and their failure to be adequately captured within the conventional  benchmarks. Finally, we propose  potential strategies to enhance generalization in text embedding models for syntactic diverse settings. This research contributes to understanding the challenges of syntactic generalization and provides valuable guidance for improving model performance in varied syntactic contexts.
\end{abstract}
